Estimating Weighted Matchings in $o(n)$ Space

We consider the problem of estimating the weight of a maximum weighted matching of a weighted graph $G(V,E)$ whose edges are revealed in a streaming fashion. We develop a reduction from the maximum weighted matching problem to the maximum cardinality matching problem that only doubles the approximation factor of a streaming algorithm developed for the maximum cardinality matching problem. Our results hold for the insertion-only and the dynamic (i.e, insertion and deletion) edge-arrival streaming models. The previous best-known reduction is due to Bury and Schwiegelshohn (ESA 2015) who develop an algorithm whose approximation guarantee scales by a polynomial factor. As an application, we obtain improved estimators for weighted planar graphs and, more generally, for weighted bounded-arboricity graphs, by feeding into our reduction the recent estimators due to Esfandiari et al. (SODA 2015) and to Chitnis et al. (SODA 2016). In particular, we obtain a $(48+\epsilon)$-approximation estimator for the weight of a maximum weighted matching in planar graphs.

==> applications.tex <==
\section{Applications}
\label{sec:applications}

\subsection{Graphs with Bounded Arboricity in Insertion-Only Streaming}
First, we focus on graphs with bounded arboricity. A graph $G=(V,E)$ has arboricity $\nu$ if
\[\nu=\max_{U\subseteq V}\left\lceil\frac{|E(U)|}{|U|-1}\right\rceil\enspace,\]
where $E(U)$ is the subset of edges with both endpoints in $U$. The class of graphs with bounded arboricity includes several important families of graphs, such as planar graphs, or more generally, graphs with bounded degree, genus, or treewidth.

Esfandiari, et al. \cite{EsfandiariHLMO15} provide an estimator for the maximum cardinality matching in the insertion-only streaming model by defining and estimating values for light vertices, heavy vertices, and shallow edges:
\begin{theorem}\label{thm:arboricity:MCM:insertion}\cite{EsfandiariHLMO15}
Let $G$ be a graph with arboricity $\nu$ and $n=\omega(\nu^2)$ vertices. Let $\epsilon,\delta\in(0,1)$ be two arbitrary positive values less than one. There exists an algorithm that estimates the size of a maximum matching in $G$ within a $(5\nu+9)(1+\epsilon)^2\rceil(1+\epsilon)$-factor in the insertion-only streaming model with probability at least $(1-\delta)$, using $\tilde{\mathcal{O}}(\nu\epsilon^{-2}\log(\delta^{-1})n^{2/3})$ space.
Both the update time and final processing time are $\mathcal{O}(\log(\delta^{-1}))$.

In particular, for planar graphs, by choosing $\delta=n^{-1}$ and $\epsilon$ as a small constant, the output of our algorithm is a $24+\epsilon$-approximation of the size of the maximum matching with probability at least $1-\frac{1}{n}$ using at most $\tilde{\mathcal{O}}(n^{2/3})$ space.
\end{theorem}

Before applying Theorem \ref{thm:main}, we observe:
\begin{lemma}
\label{lem:arboricity:subgraph}
If graph $G=(V,E)$ has arboricity at most $\nu$, then subgraph $G'=(V,E')$ where $E'\subseteq E$ also has arboricity at most $\nu$.
\end{lemma}
Thus, we have:
\begin{corollary}\label{thm:arboricity}
Let $G$ be a graph with arboricity $\nu$ and $n=\omega(\nu^2)$ vertices. Let $\epsilon,\delta\in(0,1)$ be two arbitrary positive values less than one. There exists an algorithm that estimates the maximum weighted matching in $G$ within a $2\lceil(5\nu+9)(1+\epsilon)^2\rceil(1+\epsilon)$-factor in the insertion-only streaming model with probability at least $(1-\delta)$, using $\tilde{\mathcal{O}}(\nu\epsilon^{-2}\log(\delta^{-1})n^{2/3})$ space.
Both the update time and final processing time are $\mathcal{O}(\log(\delta^{-1}))$.

In particular, for planar graphs, by choosing $\delta=n^{-1}$ and $\epsilon$ as a small constant, the output of our algorithm is within $48+\epsilon$-approximation of the maximum weighted matching with probability at least $1-\frac{1}{n}$ using at most $\tilde{\mathcal{O}}(n^{2/3})$ space.
\end{corollary}
\begin{proof}
Given Lemma \ref{lem:arboricity:subgraph}, then each subgraph also falls in the class of graphs with bounded arboricity. Thus, Theorem \ref{thm:arboricity:MCM:insertion} satisfies the conditions of Theorem \ref{thm:main} with $\alpha=(5\nu+9)(1+\epsilon)^2$.

In particular, planar graphs have $\nu\le3$, which provides a $48+\epsilon$-approximation.
\end{proof}

\subsection{Graphs with Bounded Arboricity in the Dynamic Model}
Chitnis, et al. \cite{ChitnisCEHMMV16} provide an estimator for the maximum cardinality matching in the dynamic model:
\begin{theorem}\label{thm:arboricity:MCM:dynamic}\cite{ChitnisCEHMMV16}
Let $G$ be a graph with arboricity $\nu$ and $n=\omega(\nu^2)$ vertices. Let $\epsilon,\delta\in(0,1)$ be two arbitrary positive values less than one. There exists an algorithm that estimates the size of a maximum matching in $G$ within a $(5\nu+9)(1+\epsilon)^2\rceil(1+\epsilon)$-factor in the insertion-only streaming model with probability at least $(1-\delta)$, using $\tilde{\mathcal{O}}(\nu\epsilon^{-2}\log(\delta^{-1})n^{4/5})$ space.
Both the update time and final processing time are $\mathcal{O}(\log(\delta^{-1}))$.

In particular, for planar graphs, by choosing $\delta=n^{-1}$ and $\epsilon$ as a small constant, the output of our algorithm is a $24+\epsilon$-approximation of the size of the maximum matching with probability at least $1-\frac{1}{n}$ using at most $\tilde{\mathcal{O}}(n^{4/5})$ space.
\end{theorem}
Given Lemma \ref{lem:arboricity:subgraph}, then each subgraph also falls in the class of graphs with bounded arboricity. Thus, Theorem \ref{thm:arboricity:MCM:dynamic} satisfies the conditions of Theorem \ref{thm:main} with $\alpha=(5\nu+9)(1+\epsilon)^2$. Consequently, we have:
\begin{corollary}\label{cor:arboricity:dynamic}
Let $G$ be a graph with arboricity $\nu$ and $n=\omega(\nu^2)$ vertices. Let $\epsilon,\delta\in(0,1)$ be two arbitrary positive values less than one. There exists an algorithm that estimates the maximum weighted matching in $G$ within a $2\lceil(5\nu+9)(1+\epsilon)^2\rceil(1+\epsilon)$-factor in the dynamic streaming model with probability at least $(1-\delta)$, using $\tilde{\mathcal{O}}(\nu\epsilon^{-2}\log(\delta^{-1})n^{4/5})$ space.
Both the update time and final processing time are $\mathcal{O}(\log(\delta^{-1}))$.

In particular, for planar graphs, by choosing $\delta=n^{-1}$ and $\epsilon$ as a small constant, the output of our algorithm is a $48+\epsilon$-approximation of the maximum weighted matching with probability at least $1-\frac{1}{n}$ using at most $\tilde{\mathcal{O}}(n^{4/5})$ space.
\end{corollary}





\iffalse
\subsection{Bipartite Graphs}
A bipartite graph $G=(V,E)$ whose vertices can be partitioned into two disjoint sets $X$ and $Y$ so that every edge in $E$ connects a vertex in $X$ and a vertex in $Y$.
\begin{theorem}\label{thm:bipartite}
Let $G$ be a bipartite graph with maximum vertex degree $\Delta$. Let $\epsilon,\delta\in(0,1)$ be two arbitrary positive values less than one. There exists an algorithm that estimates the maximum weighted matching in $G$ within a $2\Delta(1+\epsilon)$-factor in the streaming model with probability at least $(1-\delta)$, using $\tilde{\mathcal{O}}(\Delta\epsilon^{-2}\log(\delta^{-1})n^{2/3})$ space.
Both the update time and final processing time are $\mathcal{O}(\log(\delta^{-1}))$.
\end{theorem}
\begin{lemma}
Let $G$ be a bipartite graph with maximum vertex degree $\Delta$ and maximum matching size $M^*$. We have the following bounds:
\begin{itemize}
\item
upper bound: $M^*\le|E|$,
\item
lower bound: $M^*\ge\frac{|E|}{\Delta}$.
\end{itemize}
\end{lemma}
\begin{proofof}{Theorem \ref{thm:bipartite}}
Because any subgraph of a bipartite graph with bounded degree will also be a bipartite graph with bounded degree, the proposed modification satisfies the conditions of Theorem \ref{thm:main} with $\alpha=\Delta$.
\end{proofof}

\subsection{Job Scheduling Problem}
In the \emph{vertex arrival} model, each stream update is a vertex $v$ along with all of its incident edges.
\begin{theorem}\label{thm:scheduling}
In the streaming job scheduling problem, let $J$ be the maximum number of candidate jobs which overlap, and let $T$ be the longest time for a job. Let $\epsilon,\delta\in(0,1)$ be two arbitrary positive values less than one. There exists an algorithm that estimates the maximum weighted matching in $G$ within a $\max(J,T)(1+\epsilon)$-factor in the streaming model with probability at least $(1-\delta)$, using space $\tilde{\mathcal{O}}(\max(J,T)\epsilon^{-2}\log(\delta^{-1})n^{2/3})$.
Both the update time and final processing time are $\mathcal{O}(\log(\delta^{-1}))$.
\end{theorem}
\fi
